SliderSpace: Decomposing the Visual Capabilities of Diffusion Models

We present SliderSpace, a framework for automatically decomposing the visual capabilities of diffusion models into controllable and human-understandable directions. Unlike existing control methods that require a user to specify attributes for each edit direction individually, SliderSpace discovers multiple interpretable and diverse directions simultaneously from a single text prompt. Each direction is trained as a low-rank adaptor, enabling compositional control and the discovery of surprising possibilities in the model's latent space. Through extensive experiments on state-of-the-art diffusion models, we demonstrate SliderSpace's effectiveness across three applications: concept decomposition, artistic style exploration, and diversity enhancement. Our quantitative evaluation shows that SliderSpace-discovered directions decompose the visual structure of model's knowledge effectively, offering insights into the latent capabilities encoded within diffusion models. User studies further validate that our method produces more diverse and useful variations compared to baselines. Our code, data and trained weights are available at https://sliderspace.baulab.info

==> rebuttal-figures/person_examples.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{rebuttal-figures-src/person.pdf}
    \vspace{-1.5em}
    \caption{SliderSpace directions for the ``person'' concept (top) successfully generalize to related ``police'' and ``athlete'' concepts. They also transfer to out-of-domain concepts like ``dog''}
    \vspace{-0.5em}
    \label{fig:reb-person}
\end{figure}


==> sec/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sup-figures/turbo_concept2.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{sup-figures-src/turbo_concept_bird-cropped.pdf}
    \caption{We show the SliderSpace discovered in SDXL-Turbo 4-step model~\cite{turbo} for the concept ``Bird''} 
    \label{fig:turbo2}
\end{figure*}


==> sup-figures/turbo_concept3.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{sup-figures-src/turbo_concept_castle-cropped.pdf}
    \caption{We show the SliderSpace discovered in SDXL-Turbo 4-step model~\cite{turbo} for the concept ``Castle''} 
    \label{fig:turbo3}
\end{figure*}


==> sup-figures/turbo_concept4.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{sup-figures-src/turbo_concept_temple-cropped.pdf}
    \caption{We show the SliderSpace discovered in SDXL-Turbo 4-step model~\cite{turbo} for the concept ``Temple''} 
    \label{fig:turbo4}
\end{figure*}


==> tables/art_fid.tex <==
\begin{table}
    \centering
    \begin{tabular}{rcccc}
        & & \multicolumn{2}{c}{\textbf{User Study}} \\
        \textbf{Method} & \textbf{FID} & \textbf{Diversity}  & \textbf{Utility} \\
        \hline
        Artists Prompt &  - & todo & todo \\
        Generic Prompt & 76.08 & todo & todo \\

        LLM Prompt & 38.84 & todo & todo \\

        SliderSpace (Ours) & \textbf{21.82}& todo& todo \\

    \end{tabular}
    \caption{SliderSpace extracts a larger spread of art capabilities from the model compared to using LLMs for art inspiration prompts. We measure the FID between the dataset of all artists present in the model and different baselines. Additionally, our user study, reveals that sliderspace can be more diverse and usable. \nik{TODO: convert to figure with grid per method and FID under each}}
    \label{tab:artfid}
\end{table}

==> tables/concept_dreamsim.tex <==
\begin{table}
    \centering
   \begin{tabular}{lcccc}
        % \hline
        & \multicolumn{2}{c}{\textbf{Base Model}} & \multicolumn{2}{c}{\textbf{SliderSpace}} \\
        \textbf{Concept} & \textbf{Diversity} & \textbf{CLIP} & \textbf{Diversity} & \textbf{CLIP} \\
        \hline
        Monster & 0.266  & 28.14 & 0.472  & 28.37 \\
        Mountain & 0.217  & 29.75 & 0.387  & 29.33 \\
        Person & 0.423 & 27.38 & 0.613 & 27.40 \\
        Van Gogh & 0.349  & 31.94 & 0.557  & 32.20 \\
        Cat & 0.145  & 29.95 & 0.387  & 30.20 \\
        Dog & 0.246  & 29.38 & 0.444 & 29.20 \\

    \end{tabular}
    \caption{SliderSpace enables diverse image generation as indicated by DreamSim\cite{dreamsim} distance across generated images while also having a good text-to-image alignment through CLIP scores. [Diversity - can be thought as a way to measure model's recall of diverse visual variations; CLIP - can be thought as measuring precision of the model's output by evaluating how relevant the images are to the prompt used.]}
    \label{tab:dreamsim}
\end{table}
